3D Reconstruction of Novel Object Shapes from Single Images

Accurately predicting the 3D shape of any arbitrary object in any pose from a single image is a key goal of computer vision research. This is challenging as it requires a model to learn a representation that can infer both the visible and occluded portions of any object using a limited training set. A training set that covers all possible object shapes is inherently infeasible. Such learning-based approaches are inherently vulnerable to overfitting, and successfully implementing them is a function of both the architecture design and the training approach. We present an extensive investigation of factors specific to architecture design, training, experiment design, and evaluation that influence reconstruction performance and measurement. We show that our proposed SDFNet achieves state-of-the-art performance on seen and unseen shapes relative to existing methods GenRe and OccNet. We provide the first large-scale evaluation of single image shape reconstruction to unseen objects. The source code, data and trained models can be found on https://github.com/rehg-lab/3DShapeGen.

==> figures/quantitative_comparison.tex <==

\begin{figure*}

\begin{minipage}{.45\linewidth}
\centering
\begin{table}[H]
\input{tables/method_comp_genre_data}
\caption{SDFNet outperforms GenRe~\cite{genre} on 9 unseen classes of the data split released by~\cite{genre}. We report CD since this is the sole evaluation metric used by GenRe.}
\label{table:method_comparison_genre_data}
\end{table}
\end{minipage}
\hspace{5pt}
\centering
\begin{minipage}{0.45\linewidth}
\centering
\begin{table}[H]
\input{tables/method_comparison}
\caption{SDFNet outperforms prior work on seen and unseen classes of 2-DOF ShapeNet testing data, using four commonly used evaluation metrics with a focus on FS@1. IoU is omitted for GenRe as per the authors' recommendation since the meshes are not guaranteed to be wateright.}
\label{table:method_comparison}
\end{table}
\end{minipage}




\end{figure*}

\begin{comment}
\begin{minipage}{.3\linewidth}
\centering
\includegraphics[height=9cm]{figures/rep_viz.pdf}
\caption{Visualization of output meshes from seen and unseen categories with 3-DOF ShapeNet testing. The 3-DOF VC model has the best reconstruction quality for novel shapes in arbitrary poses.\SSnote{this layout is not as good as I thought it would be. Will fix}}
\end{minipage}
\end{comment}
